Chit-Chat or Deep Talk: Prompt Engineering for Process Mining

This research investigates the application of Large Language Models (LLMs) to augment conversational agents in process mining, aiming to tackle its inherent complexity and diverse skill requirements. While LLM advancements present novel opportunities for conversational process mining, generating efficient outputs is still a hurdle. We propose an innovative approach that amend many issues in existing solutions, informed by prior research on Natural Language Processing (NLP) for conversational agents. Leveraging LLMs, our framework improves both accessibility and agent performance, as demonstrated by experiments on public question and data sets. Our research sets the stage for future explorations into LLMs' role in process mining and concludes with propositions for enhancing LLM memory, implementing real-time user testing, and examining diverse data sets.

==> Makefile <==
# LATEX: pdflatex | xelatex | lualatex
LATEX = lualatex
LATEX_FLAGS = -shell-escape
BIBTEX = bibtex

FILES = $(patsubst %.tex, %.pdf, $(wildcard *.tex))

all: $(FILES)


%.pdf: %.tex
	$(LATEX) $(LATEX_FLAGS) $<
	$(LATEX) $(LATEX_FLAGS) $<
	-$(BIBTEX) `basename $< .tex`
	$(LATEX) $(LATEX_FLAGS) $<
	$(LATEX) $(LATEX_FLAGS) $<
	$(LATEX) $(LATEX_FLAGS) $<
	qpdf --linearize --newline-before-endstream $@ /tmp/$@
	mv /tmp/$@ $@

clean:
	-rm -f *.{log,toc,tac,aux,dvi,ps,bbl,blg,tmp,nav,out,snm,vrb,rel,cut,abs,xmpi,xmpdata,*~}
	-rm -rf out _minted* auto
	for i in $(ALLSUBDIRS); do \
	    (cd $$i; make clean) || exit 1; \
	done
	-rm $(FILES)

cleanall: clean
	-rm -rf out auto

==> bib.tex <==

%
% ---- Bibliography ----
%
\begin{thebibliography}{5}

\bibitem{reinkemeyer} Reinkemeyer, Lars. "Process mining in action." Process Mining in Action Principles, Use Cases and Outloook (2020).

\bibitem{brown} Brown, Tom, Benjamin Mann, Nick Ryder, Melanie Subbiah, Jared D. Kaplan, Prafulla Dhariwal, Arvind Neelakantan et al. "Language models are few-shot learners." Advances in neural information processing systems 33 (2020)

\bibitem{barb1} Barbieri, Luciana, Edmundo Roberto Mauro Madeira, Kleber Stroeh, and Wil MP van der Aalst. "Towards a natural language conversational interface for process mining." In Process Mining Workshops: ICPM 2021 International Workshops, Eindhoven, The Netherlands, October 31–November 4, 2021, Revised Selected Papers, pp. 268-280. Cham: Springer International Publishing, 2022.

\bibitem{dongen} van Dongen, B.F., Dataset BPI Challenge 2019. 4TU.Centre for Research Data. 
https://doi.org/10.4121/uuid:d06aff4b-79f0-45e6-8ec8-e19730c248f1

\bibitem{aalst} van der Aalst, Wil MP. "Process mining: a 360 degree overview." In Process Mining Handbook, pp. 3-34. Cham: Springer International Publishing, 2022.

\bibitem{johnson} Johnson, Douglas, Rachel Goodman, J. Patrinely, Cosby Stone, Eli Zimmerman, Rebecca Donald, Sam Chang et al. "Assessing the accuracy and reliability of AI-generated medical responses: an evaluation of the Chat-GPT model." (2023).

\bibitem{brocke} vom Brocke, Jan, Mieke Jans, Jan Mendling, and Hajo A. Reijers. "A five-level framework for research on process mining." Business \& Information Systems Engineering (2021): 1-8.

\bibitem{martin} Martin, Niels, Jochen De Weerdt, Carlos Fernández-Llatas, Avigdor Gal, Roberto Gatta, Gema Ibáñez, Owen Johnson et al. "Recommendations for enhancing the usability and understandability of process mining in healthcare." Artificial Intelligence in Medicine 109 (2020): 101962.

\bibitem{kubrak} Kubrak, Kateryna, Fredrik Milani, and Alexander Nolte. "A visual approach to support process analysts in working with process improvement opportunities." Business Process Management Journal 29, no. 8 (2023): 101-132.

\bibitem{dumas:fourn} Dumas, M., Fournier, F., Limonad, L., Marrella, A., Montali, M., Rehse, J., ... \& Weber, I. Augmented business process management systems: a research manifesto. CoRR abs/2201.12855 (2022).


\bibitem{merav} Allouch, Merav, Amos Azaria, and Rina Azoulay. "Conversational agents: Goals, technologies, vision and challenges." Sensors 21, no. 24 (2021): 8448.
\bibitem{vanderaa} Van der Aa, Han, Josep Carmona Vargas, Henrik Leopold, Jan Mendling, and Lluís Padró. "Challenges and opportunities of applying natural language processing in business process management." In COLING 2018: The 27th International Conference on Computational Linguistics: Proceedings of the Conference: August 20-26, 2018 Santa Fe, New Mexico, USA, pp. 2791-2801. Association for Computational Linguistics, 2018.

\bibitem{barb2} Barbieri, Luciana, Edmundo Madeira, Kleber Stroeh, and Wil van der Aalst. "A natural language querying interface for process mining." Journal of Intelligent Information Systems (2022): 1-30.

\bibitem{choi} Choi, Jonathan H., Kristin E. Hickman, Amy Monahan, and Daniel Schwarcz. "Chatgpt goes to law school." Available at SSRN (2023).

\bibitem{taylor} Sorensen, Taylor, Joshua Robinson, Christopher Michael Rytting, Alexander Glenn Shaw, Kyle Jeffrey Rogers, Alexia Pauline Delorey, Mahmoud Khalil, Nancy Fulda, and David Wingate. "An information-theoretic approach to prompt engineering without ground truth labels." arXiv preprint arXiv:2203.11364 (2022).

\bibitem{takeshi} Kojima, Takeshi, Shixiang Shane Gu, Machel Reid, Yutaka Matsuo, and Yusuke Iwasawa. "Large language models are zero-shot reasoners." (2022).

\bibitem{yang} Yang, Zhengyuan, Zhe Gan, Jianfeng Wang, Xiaowei Hu, Yumao Lu, Zicheng Liu, and Lijuan Wang. "An empirical study of gpt-3 for few-shot knowledge-based vqa." In Proceedings of the AAAI Conference on Artificial Intelligence, vol. 36, no. 3, pp. 3081-3089. 2022.

\bibitem{sezgin} Sezgin, Emre, Joseph Sirrianni, and Simon L. Linwood. "Operationalizing and implementing pretrained, large artificial intelligence linguistic models in the US health care system: outlook of generative pretrained transformer 3 (GPT-3) as a service model." JMIR medical informatics 10, no. 2 (2022): e32875.

\bibitem{harsha} Nori, Harsha, Nicholas King, Scott Mayer McKinney, Dean Carignan, and Eric Horvitz. "Capabilities of gpt-4 on medical challenge problems." arXiv preprint arXiv:2303.13375 (2023).



\end{thebibliography}

==> sn_approach.tex <==
\section{Architecture and process for prompt engineering}\label{approach}
%TODO: An introductory sentence to gneric approach
In this section, we will firstly outline the generic approach, including the primary challenges our solution addresses. We will then provide a brief overview of the main architecture, describing the most important element and its role within the overall framework. In the third sub-section, we will clarify the orchestration process for answering questions, highlighting the architecture components responsible for individual tasks.
\subsection{Generic approach}
One of the main challenges in implementing natural language interfaces for process mining analysis using LLMs is the creation of nuanced, context-specific task descriptions. These must generate SQL queries that are not only semantically correct but also precisely address the user's question.
A common strategy employed to address such problems entails the generation of a prompt, including the users question, followed by a request to generate SQL which answers the question. Such prompt typically includes instructions regarding the format and characteristics expected in the SQL statement. The SQL is then executed against an event log database and the resulting solution, or an error, is fed back to the system which decides whether to display it to the user or withhold it based on predefined criteria.


This approach, however, underperforms in the following scenarios: 
\begin{enumerate}
\item The question contains domain-specific terms.
    \begin{enumerate}
        \item Effect: LLM is unable to understand the specific terms and falls back to generic meaning of the words. Often this leads to incorrect interpretation of the questions and therefore answer is inappropriate.
    \end{enumerate}
\item The SQL is malformed.
    \begin{enumerate}
        \item Effect: Error in execution of SQL, the user does not see an answer.
    \end{enumerate}
\item The question is complex and requires multiple SQL statements.
    \begin{enumerate}
        \item Effect: The answer is malformed or meaningless SQL, alternatively, the generated SQL makes many assumptions and does not answer the actual question. 
    \end{enumerate}
\item The data model is not standard or LLM does not have sufficient information about its structure.
    \begin{enumerate}
        \item Effect: the LLM hallucinates column names, makes assumptions about data formatting. The ensuing SQL statements either exhibit functional inadequacies, leading to erroneous outcomes, or generate outputs characterized by nonsensical or stochastic properties.
    \end{enumerate}
\end{enumerate}
In the subsequent sections, we present an architectural framework designed to effectively address the aforementioned limitations.

\subsection{Architecture}
To illustrate the architecture of our solution, consider the following scenario: we want an LLM to translate the question "What is the main bottleneck in my process in department A?" into a SQL query. The task requires specific information to execute. Necessary elements include:

\begin{enumerate}
\item The data structure, such as the case\_concept\_name field, timestamp, or event field names.
\item Process-mining-specific information, such as the information on how the eventlog is built what is the meaning of case, activity or timestamp in that context
\item Domain-specific information, such as the interpretation of the term "process bottleneck", and instructions on how it is related to the underlying data. Also as bottleneck can mean different things such as resource or time bottleneck.
\item Dataset-specific information, such as the method for calculating duration if there are no \_start, \_end timestamps for each activity.
\item Mapping of data to domain knowledge e.g. what is the representation of department A in the given dataset
\end{enumerate}
These details can be stored in a Context Ontology Table. Context Ontology, is a dataset co-created by the Large Language Model (LLM) and experts. It consolidates domain, process-mining, and dataset-specific information to enhance LLM prompts. Comprising of common terms, data structures, and domain-data mappings, it serves as a reusable asset for diverse queries, enabling the generation of context-aware, customized prompts to guide the LLM in producing precise SQL queries.

\begin{figure}
\includegraphics[scale=0.4]{images/architecture_flat.png}
\vspace{0.0cm}
\caption{Architecture of a conversational agent for process mining }
%\caption{Architecture of a proposed framework for conversational agent for process mining }
\end{figure}
Figure 1 depicts the overall architecture of our framework. To generate a response, a customized \textit{prompt}, integrating both general guidance on output structure and specific context, is created for each query. This necessitates an update to the Eventlog \textit{DB context} (fieldnames, structure, datatypes) for each new query. The LLM then establish a list of required information and employs the \textit{context ontology} to enhance the prompt. Upon receiving the prompt, the LLM crafts an \textit{SQL query} to be run against \textit{the Eventlog in the DB}. If the execution is successful, the user is provided with a response; if it fails, the LLM is given \textit{feedback}—previous results, the SQL error, and instructions for correction. This iterative cycle continues until a satisfactory answer is achieved or a set loop limit is met.

%{images/LLM4PM_Architecture.png}


% use the \includegraphics command from the graphics package
% (N.B. put \usepackage{graphics} into your preamble then)
% for inclusion of your images. A sample call could read:
% \includegraphics{myimage}



%From the ontology and Database Context, paired with the template for query creation, a tailored prompt is created. Subsequently, the LLM receives the prompt and the user's question. The encoder converts the input data into a series of vectors, each a mathematical representation of a word in the input data. This encapsulates its semantic meaning in relation to the other words in the dataset.

%The decoder, similar to the encoder, also possesses several layers of self-attention mechanisms and feed-forward neural networks. However, the decoder incorporates an additional self-attention mechanism that focuses on specific parts of the encoder's output. This facilitates the generation of output step-by-step, considering not only the information seen thus far but also the pertinent parts of the input data.



\subsection{Conceptualizing Interaction with LLM as a Process}

In the context of process mining, conversational agents face a significant challenge: they must effectively integrate diverse skill sets and knowledge domains to optimize company-specific processes. This requires data engineering expertise for understanding data contexts, process analysis capabilities to comprehend terms like "process model," "variant," "deviations," and to identify bottlenecks and improvement opportunities. Moreover, responding to domain-specific queries may require domain expert's knowledge.
\begin{figure}
\includegraphics[width=\linewidth]{LLM.png}
% use the \includegraphics command from the graphics package
% (N.B. put \usepackage{graphics} into your preamble then)
% for inclusion of your images. A sample call could read:
% \includegraphics{myimage}
\vspace{-0.3cm}
\caption{The general process of prompt engineering. }
\end{figure}


Figure 2 illustrates the process we have developed to address the diversity of required skills and knowledge. One of the unique attributes of LLMs is their effectiveness in understanding problems when specific keywords are activated, such as "you are an experienced data engineer with expertise in databases and SQL queries (...)." By establishing a process and assigning roles to segregate duties and context, enabling the LLM to focus on its specific task, the outcomes of multiple queries present a greater specificity. In order to answer a specific question a range of different prompts has to be created in order to query different aspects of a question. 
Once the context has been established, the initial prompt to the Data Engineer can be formulated. This prompt would only contain the necessary data and would instruct the LLM to construct the SQL query and elucidate the reasoning behind the sequential steps of obtaining an answer to the user's query\footnote{ Additional prompt examples can be found at \url{https://tinyurl.com/chitchatdeeptalk}}.


The diagram in Figure 3 outlines the general process constructed in our proposed 
%conversational agent
framework.
Upon receiving a user's question, the application (orchestrator) first checks for similar questions in the database. These questions have previously been submitted to an LLM to generate embeddings for each of them. If any of these vectors show a similarity greater than 0.9 with the new question, the orchestrator verifies the success of the previous answer. If successful, the sql query is executed and answer is immediately forwarded to the user. Otherwise, the orchestrator forwards the execution to prompt creation task where the context of different perspectives of the question is assembled into one general, tailored to the question prompt.
\begin{figure}
\includegraphics[width=\linewidth]{LLM4PM.png}
% use the \includegraphics command from the graphics package
% (N.B. put \usepackage{graphics} into your preamble then)
% for inclusion of your images. A sample call could read:
% \includegraphics{myimage}
\vspace{-0.3cm}
\caption{Interaction between user and LLM as a process}
\end{figure}




Upon crafting the SQL query, it would be dispatched to the database via the orchestrator. In the event of errors, the Data Engineer prompt would be supplemented with the database's error information and executed again. Upon successful query execution, the user would receive an answer to their question. After two loops the model would be changed from GPT 3.5-turbo to GPT-4. The prompt creation modul can also receive context from the most similar questions from the database. If it is not possible to create correct answer, the orchestrator would ask the user to provide additional feedback to assist in answering the question.


